RetiJev: Fast and Source-Grounded Ophthalmic Decision Models

Ophthalmic clinical decision support requires fast, accurate, and privacy-preserving inference, yet autoregressive large language models (LLMs) incur substantial latency and computational overhead for decisions among predefined actions. We therefore investigate a decision-oriented alternative to generative reasoning. Specifically, we first introduce RetiJev-Data, a source-grounded ophthalmology corpus comprising 78,158 clinical-decision and diagnosis questions derived from articles in PubMed Central and a MeSH vocabulary covering 531 eye diseases, and 50,074 guideline-grading questions spanning 11 grading systems, along with a 24,662-question evaluation benchmark. Based on this, we develop RetiJev, a family of 0.8B-9B decision models that directly score candidate answers without autoregressive decoding. Across all model sizes, RetiJev outperforms both a 27B LLM and the commercial Jev 1.13 decision model on guideline grading by 10.4-23.0 points. RetiJev-9B further achieves the highest accuracy on clinical decisions, improving over both baselines by 5.4-6.5 points while matching them on diagnosis. It answers a case in 158 ms on one GPU, 3.5x faster than LLM generation and 470x faster than reasoning. Models are released at https://github.com/Awenbocc/RetiJev.

==> figures/teaser_options/opt_a.tex <==
% Teaser option A — scatter: time per case (log) vs peak GPU memory. Values: runs/latency (see fig_teaser.tex).
\definecolor{ours}{HTML}{2166AC}\definecolor{llm}{HTML}{D6604D}
\begin{tikzpicture}
\begin{axis}[
  scale only axis, width=0.80\linewidth, height=3.5cm,
  xmode=log, log origin=infty, xmin=40, xmax=500000, ymin=-6, ymax=64,
  xtick={100,1000,10000,100000}, xticklabels={0.1\,s,1\,s,10\,s,100\,s}, xminorticks=false,
  ytick={0,20,40,60},
  xlabel={time to answer one case (log scale)}, ylabel={GPU memory (GB)},
  label style={font=\scriptsize}, tick label style={font=\scriptsize},
  ylabel shift=-3pt, xlabel shift=-2pt,
  axis lines=left, axis line style={gray!70, -}, tick style={gray!70},
  grid=major, grid style={gray!12}, clip=false,
]
\addplot[llm, densely dashed, thick, mark=*, mark size=2.8pt, mark options={solid, draw=white, fill=llm}]
  coordinates {(247,51.4) (546,51.3) (74489,51.3)};
\addplot[ours, thick, mark=*, mark size=2.8pt, mark options={draw=white, fill=ours}]
  coordinates {(133,3.3) (136,8.0) (158,31.5)};
\addplot[ours, only marks, mark=*, mark size=2.8pt, mark options={draw=ours, fill=white, thick}]
  coordinates {(347,-0.0)};
\begin{scope}[font=\scriptsize]
\node[anchor=east, ours, inner sep=3.5pt, yshift=-1.5pt] at (axis cs:133,3.3) {0.8B};
\node[anchor=east, ours, inner sep=3.5pt, yshift=1.5pt] at (axis cs:136,8.0) {2B};
\node[anchor=east, ours, inner sep=3.5pt] at (axis cs:158,31.5) {9B};
\node[anchor=west, ours, align=left, inner sep=0pt] at (axis cs:230,18.5)
  {\textbf{\eyejev} on one GPU\\[-1pt] 0.8B: 0.13\,s, 3.3\,GB\\[-1pt] 2B: 0.14\,s, 8.0\,GB\\[-1pt] 9B: 0.16\,s, 31.5\,GB};
\node[anchor=west, ours, inner sep=3pt] at (axis cs:347,0) {\eyejev-0.8B on 8 CPU cores, 0.35\,s, no GPU};
\node[anchor=south, llm, inner sep=3pt] at (axis cs:247,51.4) {scores, 0.25\,s};
\node[anchor=north, llm, inner sep=3pt] at (axis cs:546,51.3) {generates, 0.55\,s};
\node[anchor=south, llm, inner sep=3pt] at (axis cs:74489,51.3) {reasons first, 74.5\,s};
\node[anchor=north, llm, inner sep=3pt] at (axis cs:12000,51.3) {\textbf{27B LLM}, 51\,GB};
\end{scope}
\end{axis}
\end{tikzpicture}

